ZERA: Zero-init Instruction Evolving Refinement Agent -- From Zero Instructions to Structured Prompts via Principle-based Optimization

Automatic Prompt Optimization (APO) improves large language model (LLM) performance by refining prompts for specific tasks. However, prior APO methods typically focus only on user prompts, rely on unstructured feedback, and require large sample sizes and long iteration cycles-making them costly and brittle. We propose ZERA (Zero-init Instruction Evolving Refinement Agent), a novel framework that jointly optimizes both system and user prompts through principled, low-overhead refinement. ZERA scores prompts using eight generalizable criteria with automatically inferred weights, and revises prompts based on these structured critiques. This enables fast convergence to high-quality prompts using minimal examples and short iteration cycles. We evaluate ZERA across five LLMs and nine diverse datasets spanning reasoning, summarization, and code generation tasks. Experimental results demonstrate consistent improvements over strong baselines. Further ablation studies highlight the contribution of each component to more effective prompt construction. Our implementation including all prompts is publicly available at https://github.com/younatics/zera-agent.

==> sections/3_2_prompt_composition_and_iterative_ptimization.tex <==
\subsection{Prompt Composition and Iterative Optimization}

The Meta-Cognitive Agent deterministically produces a pair $(T_{t+1}, P_{t+1})$, where:
\begin{itemize}
\item $T_{t+1}$ specifies the task and sub-task type, along with a structured task description that guides reasoning and output format, and
\item $P_{t+1}$ consists of a system prompt defining the LLM’s behavioral role and a user prompt specifying the task instruction.
\end{itemize}

This decomposition tightly aligns prompt semantics with task structure, enabling consistent and interpretable output behavior across iterations.

Unlike traditional prompt search approaches that rely on sampling or scoring large candidate sets, ZERA adopts a deterministic, feedback-driven refinement strategy. While the iterative mechanism was introduced in Section 3.1, this section highlights how each successive prompt encodes increasingly rich structural cues that reflect prior evaluation outcomes—both successful and deficient.

ZERA runs for a fixed number of refinement steps, using evaluation plateaus as a proxy for convergence. Although we currently operate with a static iteration budget (e.g., 15–20 refinement rounds), enabling adaptive convergence detection remains an important direction for future work. Techniques such as confidence-based early stopping or score variance monitoring could enhance efficiency without compromising prompt quality.
